Reconstruction of cosmic-ray muon events with CUORE

We report the in-situ 3D reconstruction of through-going muons in the CUORE experiment, a cryogenic calorimeter array searching for neutrinoless double beta ($0\nu\beta\beta$) decay, leveraging the segmentation of the detector. Due to the slow time response of the detector, time-of-flight estimation is not feasible. Therefore, the track reconstruction is performed using a multi-objective optimization algorithm that relies on geometrical information from the detector as a whole. We measure the integral flux of cosmic-ray muons underground at the {\it Laboratori Nazionali del Gran Sasso}, and find our value to be in good agreement with other experiments that have performed a similar measurement. To our knowledge, this work represents the first demonstration of 3D particle tracking and reconstruction of through-going muons with per-event angular determination in a millikelvin cryogenic detector array. The analysis performed for this work will be critical for validating the muon-related background in CUPID, a next-generation $0\nu\beta\beta$ experiment, and for follow-up studies on detector response and on delayed products induced by cosmic-ray muons.

==> AuthorList.tex <==
\author{ D.~Q.~Adams\thanksref{USC} \and C.~Alduino\thanksref{USC} \and K.~Alfonso\thanksref{LBNLNucSci,VirginiaTech} \and A.~Armatol\thanksref{LBNLNucSci} \and F.~T.~Avignone~III\thanksref{USC} \and O.~Azzolini\thanksref{INFNLegnaro} \and G.~Bari\thanksref{INFNBologna} \and F.~Bellini\thanksref{Roma,INFNRoma} \and G.~Benato\thanksref{GSSI,LNGS} \and M.~Beretta\thanksref{Milano,INFNMiB} \and M.~Biassoni\thanksref{INFNMiB} \and A.~Branca\thanksref{Milano,INFNMiB} \and D.~Brandani\thanksref{BerkeleyPhys} \and C.~Brofferio\thanksref{Milano,INFNMiB} \and C.~Bucci\thanksref{LNGS} \and J.~Camilleri\thanksref{VirginiaTech} \and A.~Caminata\thanksref{INFNGenova} \and A.~Campani\thanksref{Genova,INFNGenova} \and J.~Cao\thanksref{Fudan} \and S.~Capelli\thanksref{Milano,INFNMiB} \and L.~Cappelli\thanksref{LNGS} \and L.~Cardani\thanksref{INFNRoma} \and P.~Carniti\thanksref{Milano,INFNMiB} \and N.~Casali\thanksref{INFNRoma} \and D.~Chiesa\thanksref{Milano,INFNMiB} \and Y.~Chu\thanksref{GSSI,LNGS} \and M.~Clemenza\thanksref{INFNMiB} \and S.~Copello\thanksref{INFNPavia} \and O.~Cremonesi\thanksref{INFNMiB} \and R.~J.~Creswick\thanksref{USC} \and A.~D'Addabbo\thanksref{LNGS} \and I.~Dafinei\thanksref{INFNRoma} \and S.~Dell'Oro\thanksref{Milano,INFNMiB} \and S.~Di~Domizio\thanksref{Genova,INFNGenova} \and S.~Di~Lorenzo\thanksref{LNGS} \and T.~Dixon\thanksref{Paris-Saclay} \and D.~Q.~Fang\thanksref{Fudan} \and M.~Faverzani\thanksref{Milano,INFNMiB} \and E.~Ferri\thanksref{INFNMiB} \and F.~Ferroni\thanksref{GSSI,INFNRoma} \and E.~Fiorini\thanksref{Milano,INFNMiB,fn1} \and M.~A.~Franceschi\thanksref{INFNFrascati} \and S.~J.~Freedman\thanksref{LBNLNucSci,BerkeleyPhys,fn2} \and S.H.~Fu\thanksref{LNGS} \and B.~K.~Fujikawa\thanksref{LBNLNucSci} \and S.~Ghislandi\thanksref{MIT,GSSI,LNGS} \and A.~Giachero\thanksref{Milano,INFNMiB} \and M.~Girola\thanksref{Milano,INFNMiB} \and L.~Gironi\thanksref{Milano,INFNMiB} \and A.~Giuliani\thanksref{Paris-Saclay} \and P.~Gorla\thanksref{LNGS} \and C.~Gotti\thanksref{INFNMiB} \and P.~V.~Guillaumon\thanksref{LNGS,fn3} \and T.~D.~Gutierrez\thanksref{CalPoly} \and K.~Han\thanksref{SJTU} \and E.~V.~Hansen\thanksref{BerkeleyPhys} \and K.~M.~Heeger\thanksref{Yale} \and D.~L.~Helis\thanksref{LNGS} \and H.~Z.~Huang\thanksref{UCLA} \and M.~T.~Hurst\thanksref{Pittsburgh} \and G.~Keppel\thanksref{INFNLegnaro} \and Yu.~G.~Kolomensky\thanksref{BerkeleyPhys,LBNLNucSci} \and R.~Kowalski\thanksref{JHU} \and R.~Liu\thanksref{Yale} \and L.~Ma\thanksref{Fudan,UCLA} \and Y.~G.~Ma\thanksref{Fudan} \and L.~Marini\thanksref{LNGS} \and R.~H.~Maruyama\thanksref{Yale} \and D.~Mayer\thanksref{BerkeleyPhys,LBNLNucSci} \and M.~N.~Moore\thanksref{Yale} \and T.~Napolitano\thanksref{INFNFrascati} \and M.~Nastasi\thanksref{Milano,INFNMiB} \and C.~Nones\thanksref{Saclay} \and E.~B.~Norman\thanksref{BerkeleyNucEng} \and A.~Nucciotti\thanksref{Milano,INFNMiB} \and I.~Nutini\thanksref{INFNMiB} \and T.~O'Donnell\thanksref{VirginiaTech} \and M.~Olmi\thanksref{LNGS} \and S.~Pagan\thanksref{Yale} \and C.~E.~Pagliarone\thanksref{LNGS,Cassino} \and L.~Pagnanini\thanksref{GSSI,LNGS} \and M.~Pallavicini\thanksref{Genova,INFNGenova} \and L.~Pattavina\thanksref{Milano,INFNMiB} \and M.~Pavan\thanksref{Milano,INFNMiB} \and G.~Pessina\thanksref{INFNMiB} \and V.~Pettinacci\thanksref{INFNRoma} \and C.~Pira\thanksref{INFNLegnaro} \and S.~Pirro\thanksref{LNGS} \and E.~G.~Pottebaum\thanksref{Yale} \and S.~Pozzi\thanksref{INFNMiB} \and E.~Previtali\thanksref{Milano,INFNMiB} \and A.~Puiu\thanksref{LNGS} \and S.~Puranam\thanksref{BerkeleyPhys} \and S.~Quitadamo\thanksref{GSSI,LNGS} \and A.~Ressa\thanksref{INFNRoma} \and C.~Rosenfeld\thanksref{USC} \and B.~Schmidt\thanksref{Saclay} \and R.~Serino\thanksref{Paris-Saclay} \and A.~Shaikina\thanksref{GSSI,LNGS} \and V.~Sharma\thanksref{Pittsburgh} \and V.~Singh\thanksref{BerkeleyPhys} \and M.~Sisti\thanksref{INFNMiB} \and D.~Speller\thanksref{JHU} \and P.~T.~Surukuchi\thanksref{Pittsburgh} \and L.~Taffarello\thanksref{INFNPadova} \and C.~Tomei\thanksref{INFNRoma} \and A.~Torres\thanksref{VirginiaTech} \and J.~A.~Torres\thanksref{Yale} \and K.~J.~Vetter\thanksref{MIT} \and M.~Vignati\thanksref{Roma,INFNRoma} \and S.~L.~Wagaarachchi\thanksref{BerkeleyPhys,LBNLNucSci} \and R.~Wang\thanksref{JHU} \and B.~Welliver\thanksref{BerkeleyPhys,LBNLNucSci} \and J.~Wilson\thanksref{USC} \and K.~Wilson\thanksref{USC} \and L.~A.~Winslow\thanksref{MIT} \and F.~Xie\thanksref{Fudan} \and T.~Zhu\thanksref{BerkeleyPhys} \and S.~Zimmermann\thanksref{LBNLEngineering} \and S.~Zucchelli\thanksref{BolognaAstro,INFNBologna}
} 

\institute{ Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA\label{USC} \and Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA\label{LBNLNucSci} \and Center for Neutrino Physics, Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, USA\label{VirginiaTech} \and INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy\label{INFNLegnaro} \and INFN -- Sezione di Bologna, Bologna I-40127, Italy\label{INFNBologna} \and Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy\label{Roma} \and INFN -- Sezione di Roma, Roma I-00185, Italy\label{INFNRoma} \and Gran Sasso Science Institute, L'Aquila I-67100, Italy\label{GSSI} \and INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy\label{LNGS} \and Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy\label{Milano} \and INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy\label{INFNMiB} \and Department of Physics, University of California, Berkeley, CA 94720, USA\label{BerkeleyPhys} \and INFN -- Sezione di Genova, Genova I-16146, Italy\label{INFNGenova} \and Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy\label{Genova} \and Key Laboratory of Nuclear Physics and Ion-beam Application (MOE), Institute of Modern Physics, Fudan University,Shanghai 200433, China\label{Fudan} \and INFN -- Sezione di Pavia, Pavia I-27100, Italy\label{INFNPavia} \and Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France\label{Paris-Saclay} \and INFN -- Laboratori Nazionali di Frascati, Frascati (Roma) I-00044, Italy\label{INFNFrascati} \and Massachusetts Institute of Technology, Cambridge, MA 02139, USA\label{MIT} \and Physics Department, California Polytechnic State University, San Luis Obispo, CA 93407, USA\label{CalPoly} \and INPAC and School of Physics and Astronomy, Shanghai Jiao Tong University; Shanghai Laboratory for Particle Physics and Cosmology, Shanghai 200240, China\label{SJTU} \and Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA\label{Yale} \and Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA\label{UCLA} \and Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh, PA 15260, USA\label{Pittsburgh} \and Department of Physics and Astronomy, The Johns Hopkins University, 3400 North Charles Street Baltimore, MD, 21211\label{JHU} \and IRFU, CEA, Université Paris-Saclay, F-91191 Gif-sur-Yvette, France\label{Saclay} \and Department of Nuclear Engineering, University of California, Berkeley, CA 94720, USA\label{BerkeleyNucEng} \and Dipartimento di Ingegneria Civile e Meccanica, Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, Cassino I03043, Italy\label{Cassino} \and INFN -- Sezione di Padova, Padova I-35131, Italy\label{INFNPadova} \and Engineering Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA\label{LBNLEngineering} \and Dipartimento di Fisica e Astronomia, Alma Mater Studiorum -- Universit\`{a} di Bologna, Bologna I-40127, Italy\label{BolognaAstro} 
}

\thankstext{fn1}{Deceased} \thankstext{fn2}{Deceased} \thankstext{fn3}{Presently at: Instituto de Física, Universidade de São Paulo, São Paulo 05508-090, Brazil}
